A Probabilistic Formulation of the Diffusion Coefficient in Porous Media as Function of Porosity

We investigate the upscaling of diffusive transport parameters as function of pore scale material structure using a stochastic framework. We focus on sub-REV (representative elementary volume) scale where the complexity of pore space geometry leads to a significant scatter of transport observations. We study a large data set of sub-REV measurements on porosity and transport ability being a dimensionless parameter representing the ratio of diffusive flow through the porous volume and through an empty volume. We characterize transport ability as probability distribution functions (PDFs) of porosity capturing the effect of pore structure differences among samples. We then investigate domain size effects and predict the REV scale. While scatter in porosity observation decrease linearly with increasing sample size, the observed scatter in transport ability converges towards a constant value larger zero. Our results confirm that differences in pore structure topology impact transport parameters at all scales. Consequently, the use of PDFs to describe the relationship of effective transport coefficients to porosity is advantageous to deterministic semi-empirical functions. We discuss the consequences and advocate the use of PDFs for effective parameters in both continuum equations and data interpretation of experimental or computational work. We believe that the presented statistics-based upscaling technique of sub-REV microscopy data provides a new tool in understanding, describing and predicting macroscopic transport behavior of micro-porous media.

==> Archive/Notes_done.tex <==
% \title{Upscaling Diffusive Transport in Terms of Porosity Statisitcs}
% \authors{Alraune Zech, Matthijs de Winter}

\section*{Abstract}

Gas diffusion is the rate limiting transport mechanisms in fields such as preparative chromatography and heterogeneous catalysis. The transport rate is limited by the available pore space, in particular at low porosities. Typically, pores facilitating diffusion are of the order of 1 nm up to several micrometers in diameter, which require sophisticated visualization techniques such as electron microscopy to be able to decipher the pore space. Resolving the pore space with high spatial resolution has the disadvantage that it can only probe small volumes, often below a representative elementary volume (REV). Meanwhile, heterogeneity of the pore space may occur across larger length scales.
We have investigated the statistics of transport abilities of volumes smaller than a REV as a function of porosity and percolation probability. The initial statistics are based on a fluid catalytic cracking particle. We determined a probability distribution function for the transport ability as a function of porosity. Furthermore, we investigated the effect of upscaling the probability distribution function, with special focus on sub-REV volumes. The analytical results are compared to pore network-type simulations. 
We believe that the statistics-based up-scaling technique of sub-REV microscopy data provides a new tool in understanding macroscopic transport behavior of micro-porous materials.

% When diffusion is the critical transport process, the effective diffusion parameter expresses the transport ability of the porous material. Particularly for catalyst particle, this quantity determines its overall performance.
% The scale where diffusive transport is of interest is usually larger then the scale of measurements of porosity. Thus, upscaling of transport parameters is required. However, results for the mean behavior are not sufficient when deviations from the mean are still significant. This is particularly important when porosities are close to the percolation threshold.
% We investigate the statistical behavior of the transport ability (as characteristic parameter for diffusive transport) as function of porosity statistics and percolation. We perform step-wise upscaling providing not only mean values but probability density functions. We test the procedure for data from catalytic particle where porosity measurements and their statistics are available at different scales. 

\section{Introduction}

\textbf{Abbreviations:}
\begin{itemize}
    \item porosity  $\epsilon$ or total porosity $\epsilon_\mathrm{total}$
    \item measured mean and standard deviation of porosity at resolution $n$: $\bar\epsilon^{(n)}$, $s\epsilon^{(n)}$
    \item percolating porosity:  $\varepsilon_\mathrm{perc}$  
    \item transport resistance: $tr$
    \item transport ability: $ta$ as inverse of transport resistance: $tr = 1/ta$
    \item normal distribution $N(\mu,\sigma)$ to statistical distribution parameters mean $\mu$ and standard deviation $\sigma$
    \item log-normal distribution $LN(\mu,\sigma)$ to statistical distribution parameters $\mu$ and $\sigma$ (which can be associated to mean and standard deviation of log-transformed data which follow a normal distribution)
\end{itemize}

\section{Data Analysis on Porosity and Transport Ability}

\subsection{Statistical Analysis of Total Porosity Data}
\begin{itemize}
    \item starting point: measured porosity distributions in FCC particles at different resolutions
    \item mean of porosity quasi constant, standard deviation decreasing with increasing resolution size $n$ [$\mu$m] :
    \begin{tabular}{l| c c c}
         FCC2   &   2x2 & 8x8  & 32x32   \\
         \hline
         mean $\bar\epsilon^{(n)}$                   & 0.296 & 2.9 & 2.8 \\  
         standard deviation $s\epsilon^{(n)}$     & 0.145 & 0.09 & 0.044  
%         FCC1   &   2x2 & 8x8  & 32x32   \\
%         \hline
%         mean $epsilon_m$                   & 0.241 & 2.39 & 2.39 \\  
%         standard deviation $epsilon_s$     & 0.074 & 0.048 & 0.001  
    \end{tabular}
    \item the non-zero standard deviation for porosity measurements at small resolutions indicates clearly that the domain size has not yet reached the REV level.
    \item porosity follows truncated Normal distribution: $ P(\epsilon)\propto N(\bar\epsilon^{(n)},s\epsilon^{(n)})$
    \begin{equation} \label{eq:eps_normal}
        P(\epsilon=x)=g(x,\bar \epsilon,s\epsilon)=\frac{1}{s\epsilon\sqrt{2\pi}} \exp{\left(-\frac{(x-\bar\epsilon)^2}{2 s\epsilon^2}\right)}
    \end{equation}
    to parameters mean $\bar\epsilon^{(n)}$ and standard deviation $s\epsilon^{(n)}$ according to observations (Table). pdf is truncated normal distribution for valid porosity value in the range of $[0,1]$.
    \item Figure~\ref{fig:porosity} shows truncated normal distribution of porosity for one particle at smallest resolution (tabulated values for $n=2$).
    \item porosity pdf means that the chance of measuring a certain porosity value $\epsilon_0$ for a volume of the specific resolution $n$ is given with the probability $P(\epsilon=\epsilon_0)=p$ drawn from a normal distribution with parameters~$\bar\epsilon^{(n)}$ and $s\epsilon^{(n)}$. For large resolutions $n$, the standard deviation is small and thus the porosity distribution is narrow around the mean. For small resolutions, the larger standard deviation leads to a broader range of values, covering a range from $0$ to $0.7$, however with lower chances for values far from the mean.
    \item application of law of large numbers and central limit theorem (general):
        \begin{itemize}
            \item porosity observation at every resolution can be interpreted as independent and identically distributed random variables $X_i^n$
            \item average at next higher resolution level can be defined as sum over samples at smaller resolution: $1/N S_N = 1/N \sum_i X_i$ with $N=(n_2/n_1)^2$, e.g. $n_1=2 \rightarrow n_2=8$, results in $N=4*4=16$ sub-samples
            \item central limit theorem: normalized sample average converges towards normal distribution with zero mean and variance of $X_i$ scaled by $\sqrt{N}$.
            \item standard deviation at higher resolution: $STD(1/N S_N) = 1/\sqrt{N} STD (X_i)$, which means the standard deviation converges to zero for increasing sample size at a rate of $\sqrt{N}$
        \end{itemize}
    \item application of central limit theorem to observed porosities:
        \begin{itemize}
            \item expectation value, being the mean $\bar\epsilon^{(n)}$ follows prediction: $E(1/N S_N) = E (X_i)$, since $\bar\epsilon^n$ are quasi the same for all $n=2,8,32$.
            \item standard deviation: the theoretical convergence rate of the standard deviation would be $\sqrt{N} = n_2/n_1 = 4$ ($2 \rightarrow 8  \rightarrow 32)$ whereas the observed convergence rate is roughly $2$ ( $s\epsilon^2 \approx 2 s\epsilon^8 \approx 4 s\epsilon^{32}$).
            \item possible explanation: samples are not independent, but spatially correlated (giving a slower convergence of the standard deviation to zero)
        \end{itemize}
\end{itemize}

\begin{figure}
\centering
    \includegraphics[width=0.7\textwidth]{Figures/Porosity_n2.png}
\caption{Statistical analysis of measured porosities at smallest resolution ($n=2\,\mu$m). Probability density function (pdf) of total porosity $P(\epsilon_\mathrm{total})=N(\bar\epsilon^{(n=2)}$, $s\epsilon^{(n=2)})$. Percolation probability $p_\mathrm{perc} = f(\epsilon_\mathrm{total}) \in [0,1]$, relative percolating porosity $P(\epsilon_\mathrm{total})\cdot p_\mathrm{perc}$ and pdf of percolating porosity $P(\epsilon_\mathrm{perc})=P(\epsilon_\mathrm{total})\cdot p_\mathrm{perc}(\epsilon_\mathrm{total}) / \mathrm{TPP}$ where $\mathrm{TPP}$ is the total percolating porosity.}
    \label{fig:porosity}
\end{figure}

\subsection{Statistical Analysis of Percolation as Function of Porosity}
\begin{itemize}
    \item transport ability is a function of percolation of a volume:    
        \begin{itemize}
            \item non-percolating: transport ability is zero (no transport through volume possible), thus infinite large transport resistance
            \item percolating: transport ability is non-zero, thus finite transport resistance
        \end{itemize}
    \item percolation can be statistically described using a Bernoulli distribution with $X$ being the event of percolation:
    \begin{itemize}
            \item $X=0$: non-percolating
            \item $X=1$: percolating
        \end{itemize}
    \item the probability for a volume to percolate is given by $p_\mathrm{perc} \in [0,1]$ with
        \begin{itemize}
            \item  $P(X=1)=p_\mathrm{perc}$ 
            \item $P(X=0)=1-p_\mathrm{perc}$
        \end{itemize}
    \item percolation probability $p_\mathrm{perc}=f(\epsilon)$ is assumed to be a function of porosity $\epsilon$: 
    \item analysis of data revealed polynomial functional relation between percolation probability and porosity $p_\mathrm{perc}=P(\epsilon=x)=f(x) \in [0,1]$ as given in Figure~\ref{fig:porosity}:
    \begin{equation}\label{eq:percprob}
            f(x) = 
            \begin{cases}
                    0  & \text{for } x \leq 0.07\\
                    c_3x^3+c_2x^2+c_1x+c_0 & \text{for }  0.07 < x < 0.39 \\
                    1  & \text{for } 0.39 \leq x
            \end{cases}
    \end{equation}
    \item volumes with a porosity value $\epsilon<0.07$ are considered as non-percolating ($p_\mathrm{perc}=0$), whereas volumes with large porosities $\epsilon>0.39$ are percolating ($p_\mathrm{perc}=1$); values in between follows a third order polynomial derived from a fit to the data with $c_3=27.362$, $c_2=-27.661$, $c_1=9.4256$, and $c_0=-0.0927$
    \item we can calculate the total percolating porosity (TPP) and the total amount of non-percolating porosity (TNPP) by combining the normal distribution for porosity $P(\epsilon) \propto N(\bar\epsilon^{(n)},s\epsilon^{(n)})$ and the percolation probability $p_\mathrm{perc} (\epsilon)$ by as:
        \begin{align} \label{eq:TPP}
            \mathrm{TPP}      &   = \int_0^1 P(\epsilon = x)\cdot p_\mathrm{perc} (\epsilon=x) dx = \int_0^1 g(x,\bar \epsilon, s\epsilon) \cdot f(x) dx \\
            \mathrm{TNPP}     &   = 1 - \mathrm{TPP}
        \end{align}
    \item TPP and TNPP are solely functions of the porosity statistical parameters $\bar\epsilon^{(n)}$ and $s\epsilon^{(n)})$
    \item TPP and TNPP characterize the proportion of the void space which are active in the transport process (TPP) and the part which is void but not available (TNPP), e.g. dead-end pores. These are the statistically predicted values for a domain containing sufficiently many sub-samples of porosity within, which are assumed to follow the outlined distributions.
    \item The TNPP will be close to zero when the standard deviation of porosity is small and the mean is not to close to the percolation threshold, also when the mean porosity is significantly higher then 0.39 [$p_\mathrm{perc}=f(0.39 \leq x)=1$] the amount of non-percolating volume is low.
\end{itemize}

\subsection{Transport Ability and Percolating Porosity}
\begin{itemize}
    \item again, in a first step transport ability as function of porosity depends on the percolation:
    \begin{equation}%\label{ta_per}
            ta(\epsilon) = 
            \begin{cases}
                    0  & \text{ with } 1-p_\mathrm{perc}(\epsilon) \text{  (} \epsilon \text{ is non-percolating)}\\
                    ta_\mathrm{perc} \neq 0 & \text{ with } p_\mathrm{perc}(\epsilon) \text{  (}  \epsilon \text{ percolating)}
            \end{cases}
    \end{equation}
    \item focusing on percolating volumes, then transport ability $ta$ is generally not deterministic, but follows again a distribution $D(a_1,a_2,...)$ where $a_i$ are the parameter of the distribution $D$.
    \item the dependency of $ta$ as function of percolating porosity is then expressed in the input parameter of $D$ being functions of $\varepsilon_\mathrm{perc}$: $a_1(\varepsilon_\mathrm{perc})$, $a_2(\varepsilon_\mathrm{perc})$
    \item Before focusing on the distribution of $ ta_\mathrm{perc}$ as function of percolating porosity we have a closer look on the percolating porosity.
    \item the percolating porosity $\epsilon_\mathrm{perc}$ is defined as a subset of all porosity values, specifically those which percolate; regard $P(\epsilon = \epsilon_\mathrm{perc}) =  p_\mathrm{perc}(\epsilon) = f(\epsilon_\mathrm{perc})$
    \item the percolating porosity is a function of the statistical parameters of the porosity $\bar\epsilon^{(n)}$, $s\epsilon^{(n)}$. 
    \item the distribution function for the percolating porosity $\epsilon_\mathrm{perc}$ (based on the total porosity statistical parameters ($\bar \epsilon,s\epsilon$) is then given by $P(x=\epsilon_\mathrm{perc})= P(x=\epsilon_\mathrm{total})\cdot p_\mathrm{perc}(x=\epsilon_\mathrm{total}) = g(x,\bar \epsilon, s\epsilon) \cdot f(x) $. It becomes a pdf when normalizing, thus dividing by $\mathrm{TPP}$.
    \item Figure~\ref{fig:porosity} shows the percolating porosity pdf in relation to the total porosity pdf and the percolation probability for porosity parameters of mean and standard deviation as measured for the FCC2 at resolution $n=2\mu$m. 
    Here, the amount of percolating porosity is $\mathrm{TPP}=85.2\%$. Thus, about $15\%$ of the void volume does not contribute to transport being non-percolating, having a transport ability of $0$.
\end{itemize}
%\bar\epsilon^{(n)}$, $s\epsilon^{(n)}$
%\textbf{Transport Ability for Total Porosity}
%\item Experimental results indicated a log-normal distribution of $ta_\mathrm{perc}$ for percolating porosity $\epsilon_perc$ (details follow later)
    % \item The probability of transport ability can then be expressed by:
    % \begin{equation}%\label{ta_per}
    %         ta(\epsilon) = 
    %         \begin{cases}
    %                 0  & \text{ with } 1-p_\mathrm{perc}(\epsilon) \\
    %                 ta_\mathrm{perc} \neq 0 & \text{ with } p_\mathrm{perc}(\epsilon) \text{  (}  \epsilon \text{ percolating)}
    %         \end{cases}
    % \end{equation}


\begin{figure}
\centering
    \includegraphics[width=0.7\textwidth]{Figures/Scatter_TA_Data.png}
\caption{Scatter plot of transport ability (reciprocal to transport resistance) as function of percolating porosity from simulations (Data paper).}
    \label{fig:scatter}
\end{figure}

\begin{figure}
\centering
    \includegraphics[width=0.45\textwidth]{Figures/Normality_Histogram_016.png}
    \includegraphics[width=0.45\textwidth]{Figures/Normality_Histogram_034.png}
\caption{Statistical analysis of transport ability for individual percolating porosity values: Frequency distribution of data (in green) in normal (top) and log-scale (bottom) in comparison to normal (orange line) and log-normal (red line) distribution. Normality tests of Shapiro, D'Agostino and Darling-Anderson with 0 not normal and 1 normal for a significance level of $\alpha=5\%$.}
    \label{fig:stats_normal}
\end{figure}


\subsection{Statistical data analysis of transport ability for percolating porosity values}
\begin{itemize}
    \item we now investigate the transport ability $ta$ as function of porosity (given that this is a percolating porosity) and its stochastic distribution.
    \item \cite{deWinter16} determined the statistical behaviour of the transport resistance $tr=1/ta$ (as the inverse of transport ability) for smallest spatial resolution of $n=2\,\mu$m using numerical analog models.
    \begin{itemize}
        \item Figure~\ref{fig:scatter} summarized the observed transport abilities as function of (percolating porosity) in scatter plot
        \item binning the data for percolating porosities at bin levels of $0.02$ provides data distributions of $ta$ as function of $\varepsilon$ (being the bin center). 
        \item technical note: only further analysis of bins with $n>20$ values of $ta$ and for porosities above percolation threshold $\varepsilon_\mathrm{perc}\geq 0.07$
    \end{itemize}
    \item Figure~\ref{fig:stats_normal} shows the pdf's of transport ability  as function of two selected ranges of $\varepsilon_\mathrm{perc}$ by binning of data for percolating porosity values at bin levels of $0.02$ 
    \item Statistical hypothesis testing of $ta(\varepsilon_\mathrm{perc})$-pdf on normality and log-normality:
        \begin{itemize}
            \item classical hypothesis tests on normality: Shapiro-Wilk Test, D’Agostino’s  Test and Anderson-Darling Test at significance level of $\alpha=5\%$
            \item tests indicated that $ta$-pdfs can be considered log-normal distributed for small values of porosity $\varepsilon_\mathrm{perc}<0.2$
            \item transport abilities for percolating porosities around the input mean porosity $\varepsilon_\mathrm{perc} \approx \bar \epsilon \approx 0.3$ give positive outcomes in the normality test, but also agree with the log-normal distribution. 
            \item for large values of porosity, the transport ability values scatter very strongly towards small values of transport ability not giving positive outcomes of the normality tests for neither scales.
            % \item application of tests versus log-$tr$ data indicated normality of small $\varepsilon_\mathrm{perc}<0.18$ , but only partially for larger~$\varepsilon_\mathrm{perc}$
            % \item all tests indicated that $ta$-pdfs are mostly normal distributed for all values of porosity
            \item visual comparison of data indicated acceptable agreement of data and log-normal distribution
            \item Summary of statistics for two values of percolating porosity $\varepsilon_\mathrm{perc}$ given in Figure~\ref{fig:stats_normal}
        \end{itemize}
    \item conclusion that $ta$ is log-normal distributed $P_{tr}(\varepsilon_\mathrm{perc})=LN(\mu (\varepsilon_\mathrm{perc}),\sigma(\varepsilon_\mathrm{perc}))$ with distribution parameters as functions of $\varepsilon_\mathrm{perc}$; log-normal distribution parameter $\mu$ and $\sigma$ can be associated to the mean and the standard deviation of the log-$ta$ data (being a characteristic of log-normal distribution)
    \item Figure~\ref{fig:pdf_param_fit} shows the log-normal distribution parameters $\mu$ and $\sigma$ as function of $\varepsilon_\mathrm{perc}$:
    \begin{itemize}
        \item log-ta mean $\mu(\varepsilon_\mathrm{perc})$ shows a linear or slightly quadratic relationship; standard deviation is high  $\sigma(\varepsilon_\mathrm{perc})$ for small porosities and decreases with increasing porosity with highest values for porosities between $0.2$ and $0.3$ being well approximated by a cubic fit:
        \item polynomial fit: (Figure~\ref{fig:pdf_param_fit}):
        \begin{align}\label{eq:logtrmean}
            \mu(\varepsilon_\mathrm{perc}) & = a_2 \varepsilon_\mathrm{perc}^2 + a_1 \varepsilon_\mathrm{perc} + a_0 \\
            \sigma(\varepsilon_\mathrm{perc}) & = b_3 \varepsilon_\mathrm{perc}^3 b_2 \varepsilon_\mathrm{perc}^2 + b_1 \varepsilon_\mathrm{perc} + b_0
        \end{align}
        % \item polynomial fit to linear and quadratic functions (Figure~\ref{fig:pdf_param_fit}):
        % \begin{align}\label{eq:logtrmean}
        %     \mu(\varepsilon_\mathrm{perc}) & = a_1 \varepsilon_\mathrm{perc} + a_0 \\
        %     \sigma(\varepsilon_\mathrm{perc}) & = b_2 \varepsilon_\mathrm{perc}^2 + b_1 \varepsilon_\mathrm{perc} + b_0
        % \end{align}
        % with regression estimated parameters for linear and quadratic fit: $a_0=-6.75$, $a_1=5.2$, $b_2=-2.41$, $b_1=0.935$ $b_0=0.465$ valid for a range of percolating porosities of $0.07<\varepsilon_\mathrm{perc}<0.67$.
        \item fitting parameters from regression analysis: 
        $a_2=-5.31$, $a_1=10.78$, $a_0=-5.81$, $b_3=5.7$, $b_2=-8.9$, $b_1=3.12$, $b_0=0.26$; valid for a range of percolating porosities of $0.07<\varepsilon_\mathrm{perc}<0.67$.
    \end{itemize}
    \item pdfs for transport ability as function of $\varepsilon_\mathrm{perc}$ given in Figure~\ref{fig:pdf_cloud} as statistical companion of the data scatter plot
\end{itemize}
%%% -------------------------------------------------------------------------------------%%%

\begin{figure}
\centering
    \includegraphics[width=0.7\textwidth]{Figures/Polyfit_stats_TA.png}
\caption{Distribution parameter of transport ability being log-normal distributed as function of percolating porosity: mean $\mu(\varepsilon_\mathrm{perc})$ and standard deviation $\sigma(\varepsilon_\mathrm{perc})$ of log-transformed $ta$ estimated from data (solid lines) and polynomial fits as functions of $\varepsilon_\mathrm{perc}$ with linear and quadratic fit for $\mu$ and quadratic and cubic fit for $\sigma$.}
    \label{fig:pdf_param_fit}
\end{figure}

\begin{figure}
\centering
    \includegraphics[width=0.7\textwidth]{Figures/Cloud_TA_pdf.png}
\caption{Relative distribution of transport ability log-normally distributed as function of percolating porosity to mean $\mu(\varepsilon_\mathrm{perc})$ and standard deviation $\sigma(\varepsilon_\mathrm{perc})$ according to polynomial fits. Magnitude of probability is normalized to highest value for every $\varepsilon_\mathrm{perc}$.}
    \label{fig:pdf_cloud}
\end{figure}



\subsection{Transport ability distribution for total porosity}
\begin{itemize}
    \item we combine the analysis of transport ability for percolating volumes $ta = f(\mu(\varepsilon_\mathrm{perc}),\sigma(\varepsilon_\mathrm{perc}))$ with the percolation probability $p_perc$ to have a functional relationship of transport ability to the total porosity distributed to the parameters $\bar\epsilon^{(n)}$, $s\epsilon^{(n)}$: $ta=f(\bar\epsilon^{(n)},s\epsilon^{(n)})$
    \item The pdf for the transport ability $ta$ is then given from conditional probabilities: 
    $P(ta(\epsilon) = x) = P(ta(\varepsilon_{perc})=x)\cdot p_{perc}(\epsilon) + p_{non-perc}(\epsilon)$
    its a combined pdf of the percolation (as function of porosity) and the pdf for $ta$    
        \begin{equation}%\label{ta_per}
            ta(\epsilon) = 
            \begin{cases}
                    0  & \text{ with } 1-p_\mathrm{perc}(\epsilon) \text{  (} \epsilon \text{ is non-percolating)}\\
                    ta_\mathrm{perc} \neq 0 & \text{ with } p_\mathrm{perc}(\epsilon) \text{  (}  \epsilon \text{ percolating)}
            \end{cases}
    \end{equation}

    
    \item for a given value of porosity, we start again by distinguishing between percolating and non-percolating volumes:
    \begin{itemize}
        \item the transport ability is zero for non-percolating volumes
        %; the probability of that is equal to the total amount of non-percolating porosity TNPP
        \item the transport resistance is a finite value given by the log-normal distribution $LN(\mu (\epsilon),\sigma(\epsilon))$ deduced for the percolating porosity; the probability of that is equal to the total amount of percolating porosity TPP
   \end{itemize}
   \item The pdf of $tr$ with regard to total porosity can then be expressed in the equation form:
        \begin{equation}
            P_\mathrm{tr}(\epsilon,\bar\epsilon^{(n)},s\epsilon^{(n)}) = 
            \begin{cases}
                    \infty & \text{with }  p = \mathrm{TNPP}(\bar\epsilon^{(n)},s\epsilon^{(n)}) \\
                     \\
                    LN(\mu(\epsilon),\sigma(\epsilon)) & \text{with }  p = \mathrm{TPP}(\bar\epsilon^{(n)},s\epsilon^{(n)})\\
            \end{cases}
        \end{equation}
        The probability distribution of transport ability is thus a function of the total porosity value $\epsilon$ being the input parameter for $\mu$ and $\sigma$ (Eq.~\ref{eq:logtrmean}) and the stochastic parameters $\bar\epsilon^{(n)}$ and $s\epsilon^{(n)}$, since TNPP and TPP can be calculated from Eq.~\eqref{eq:TPP}.
%        Hereby, the input parameters are functions of the total porosity value $\epsilon$ and the stochastic parameters $\bar\epsilon^{(n)}$ and $s\epsilon^{(n)}$, since TNPP and TPP can be calculated from Eq.~\eqref{eq:TPP} as well as $\mu$ and $\sigma$ from Eq.~\eqref{eq:logtrmean}.
    % \item Figure~\ref shows examples of the transport ability histogram and distribution function for two values of porosity $\epsilon$ given the porosity parameters $\bar\epsilon^{(n)}$ and $s\epsilon^{(n)}$ in the table.
%    \item given a porosity distribution of $P(\epsilon)=N()$, the percolation probability $p_\mathrm{perc} (\epsilon)$, the deduced total percolating and non-percolating porosity (TPP and TNPP, respectively) and the transport resistance for the percolating porosity, then the transport resistance for a the total porosity is
\end{itemize}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Upscaling of Transport Ability as Function of Porosity}

\subsection{Some general aspect of upscaling log-normal distributed quantities}
\begin{itemize}
    \item There exists a lot of literature on analytical expression for upscaled effective parameters for log-normal distributed values in the context of flow and pressure equations. I refer here to $K$ as hydraulic conductivity (equivalent to $ta$) and head as equivalent to pressure.
    \item assuming $K(x)$ to be spatially log-normal distributed to $p_1$ and $p_2$ (can be associated to mean and variance of normal distributed $Y=\ln K$, then the effective values in the context of uniform flow (refers to a constant pressure gradient) is a function of dimensionality $d$ and the statistical parameters $p_1$ and $p_2$:
    \begin{equation}
        K_\textup{eff} = \exp{\left( p_1 + p_2* \left( \frac{1}{2} -\frac{1}{d} \right)  \right)}        
                    = \begin{cases}
                        \exp{(p_1 - 1/2\ p_2)} = K_H & \text{for $d=1$}\\
                        \exp{(p_1)} = K_G & \text{for $d=2$}\\
                        \exp{\left( p_1 + 1/6 \ p_2\right)} & \text{for $d=3$}\\
                        \end{cases}
    \end{equation}
    with $K_H$ being the harmonic mean, $K_G$ being the geometric mean
    \item the value of $K_\textup{eff}$ increases with dimension since flow can circumvent low-$K$ areas with increasing dimension more easily giving more emphasis of larger values in the averaging process. 
\end{itemize}


\subsection{Check of standard results with numerical codes: convergence issues}
\begin{itemize}
    \item implementing the pressure equation in the context of non-uniform $K$-values is straight forward. (details?) 
    \item doing numerical checking of theoretical results requires to  generate discrete networks of log-normal distributed $K$ values. Thereby several parameters are relevant:
    \begin{itemize}
        \item statistical parameter in $K$: $p_1$ and $p_2$
        \item dimensionality: 2D and 3D 
        \item number of elements in network: $N_d = n^d$ (e.g. 10x10 values in 2D giving 100 total $K$ values)
        \item Ensemble size, meaning number of realizations of networks sharing the same statistical properties
    \end{itemize}
    \item Examples for networks with $n=10$ elements is shown in Figure ...
    \item the convergence to the theoretically predicted effective values is reached either for a large number of elements in the network or for a large number of realization (and taking the mean of them). When one realization is already showing representative behaviour then it is ergodic.
    \item the parameters are not independent: the variance value $p_2$ impacts on the number of elements in network/ensemble size to converge to effective value
\end{itemize}


\subsection{To rework: Upscaling of Transport Ability}
\begin{itemize}
    \item general aim: investigate relation between transport ability and transport resistance (being the inverse of transport ability) and porosity at scales below REV in a probabilistic manner, relationship between transport ability and porosity, upscaling behaviour of descriptive parameters
    \item starting point: observed data for input quantities
    \begin{itemize}
        \item porosity distribution parameters $\bar\epsilon^{(n)}$ and $s\epsilon^{(n)}$: mean and std (assuming porosity to follow a truncated normal distribution) as functions of spatial resolutions $n=2,8,32\,\mu$m and particle (type) 
        \item percolation probability as function of porosity value:  $p_\mathrm{perc}=f(\epsilon) \in [0,1]$, analytic expression (Eq.~\ref{eq:percprob}) assuming it to be resolution independent
        \item transport resistance pdf at smallest resolution~$n=2\mu$m:  
        $tr = LN(\mu(\varepsilon_\mathrm{perc}^{(n=2)}),\sigma(\varepsilon_\mathrm{perc}^{(n=2)}))$ as function of percolating porosity being log-normal distributed to $\mu$ and $\sigma$.
        %\item transport ability pdf for percolating porosity for smallest resolution $tr ~ LN (\mu^{(n)}(\varepsilon_\mathrm{perc}),\sigma^{(n)}(\varepsilon_\mathrm{perc}))$ with $\mu^{(n)}(\varepsilon_\mathrm{perc})$ and $\sigma^{(n)}(\varepsilon_\mathrm{perc})$ being the statistical distribution parameter for the log-normal distribution.
    \end{itemize}
    \item specific aim: 
    \begin{itemize}
        \item determine transport resistance $tr$ pdf for larger resolutions $tr (n) ~ LN(\mu(\varepsilon_\mathrm{perc}^{(n)}),\sigma(\varepsilon_\mathrm{perc}^{(n)}))$ as function of porosity distribution at that resolution ($n=8$ or $n=32$) making use of transport ability at sub-scale $n=2$.
        \item determine  transport resistance distribution parameters (mean and std of log-data $\mu^{(n)}$ and $\sigma^{(n)}$) based on porosity distribution parameter (mean and variance $\bar\epsilon^{(n)}$ and $s\epsilon^{(n)}$)
        \item determine upscaling behaviour of distribution parameters for $tr$ pdf (log-tr mean and variance)
    \end{itemize}
    \item hypothesis: upscaling of transport ability pdf parameter (PPT, $\mu(\varepsilon_\mathrm{perc})$, $\sigma(\varepsilon_\mathrm{perc})$)
        \begin{itemize}
            \item PPT converges towards 1 with increasing volume due to convergence of porosity variance towards zero (assuming mean porosities at large scale is above percolation threshold $\epsilon>0.07$). Thus no distinction between percolating and non-percolating volumes is necessary.
            \item $\mu(\varepsilon)$ is scale independent, being a linear relationship of log-tr to (percolating) porosity 
            \item $\sigma(\varepsilon)$ is not converging but to a non-zero threshold standard deviation: assumption that transport ability is in non-deterministic but probabilistic relation to porosity independent of scale.
            
            %\item $mean \mu(\varepsilon_\mathrm{total})$ is scale independent or convergent 
            
            \item standard deviation:
        \end{itemize}
\end{itemize}


==> Archive/Outline.tex <==
\section{Problem Specification}

%%% Theory
\subsection{Statistical Description of Transport Ability as Function of Porosity}
\begin{itemize}
    \item Two step approach to provide probabilistic description of $ta$ values as function of porosity $\theta$: 
    \begin{itemize}
        \item not connected: $ta = 0$ since no transport through volume possible, thus infinite large transport resistance $tr = \infty$
        \item connected: $ta \neq 0$ transport ability is non-zero, following a stochastic description with parameters being functions of porosity (finite transport resistance)
    \end{itemize}
    \item connectivity statistically described using Bernoulli distribution:
    \begin{itemize}
            \item $ta=0$ with $1- p_\textup{con}(\theta)$ (non-connected)
            \item $ta \neq 1$ with $p_\textup{con}(\theta)$ (connected)
        \end{itemize}
        Probability of connectivity $p_\textup{con}(\theta)$ is statistically dependent of porosity $\theta$
    \item for connected volumes we assume that $ta$-values follow a stochastic function $g_\theta(ta)$
    \item the general probability distribution for $ta$ follows as:
        \begin{equation}\label{eq:percprob}
            P_\theta(ta = x) = 
            \begin{cases}
                    p_\mathrm{con}(\theta) \cdot g_\theta(x)  & \text{for } x > 0\\
                    1- p_\mathrm{con}(\theta) & \text{for }  x = 0
            \end{cases}
    \end{equation}
    the second case follows from conditional probability theory.
    \item we aim to determine $P_\theta(ta = x)$ by specifying its components for the smallest resolution $n = 2\mu m$ from data: analysis of porosities, connectivity analysis of analog volumes and measured transport abilities form analog volumes
    \item the same function descriptions are applied at larger scales and their performance is validated in comparison to numerical results
\end{itemize}




==> Archive/Text_done.tex <==

\section{Introduction}
Matthijs

\section{Research Question}
 \begin{itemize}
    \item define Transport Ability
    \item TA as function of material (structure) and scale
    \item aspect REV and sub-REV limitation
    \item upscaling approach in general
%     \item derive relationship of permeability (transport ability) as function of porosity (taking percolation and not ergodicity into account), provide insight for mean and deviation behaviour 
 \end{itemize}

\section{Data and Methods}

\subsection{Porosity Observations}
\begin{itemize}
    \item material aspects, background catalytic particles, shortly scanning procedure (reference to details in other paper)
    \item data indicates Normal distribution: equation
    \item statistical parameters, particularly std is scale dependent - Figure of distribution for three scales
    \item stochastic expectation for independently distributed elements would be reduction of std according to $\sigma_{2\mu m} = 1/4 \sigma_{8\mu m}$. (square root of number of lumped samples)
    \item data reveals slower reduction of factor 2 for every areal increase step - strong indication for spatial correlation of porosity values
    \item spatial correlation of porosity has to be accounted for in upscaling
\end{itemize}

\subsection{Transport Ability}
\begin{itemize}
    \item transport ability analysed for sampling scale $2 \mu m$
    \item creation of virtual domains sharing the same structural properties as material (reference to paper)
    \item (a) analysis of connectivity: 
        \begin{itemize}
            \item Bernoulli distributed (yes/no) with probability depending on porosity: $p_{con}(\theta)$
            \item analysis of data provides functional relation for $p_{con}(\theta)$: $f(\theta) = ...$; polynomial fit (refer to paper MdW); Figure
            \item realistic representation given that decreasing porosity lowers probability of having a void space path through domain.
            \item connectivity in combination with porosity often refered to as "effective" or "connected" porosity. 
            \item over total range of porosity values this leads to portion of non-connected elements, e.g. for porosity distribution of Figure ... the shaded area refer to non-connected porosity, summing up to $...\%$.
        \end{itemize}
    \item (b) analysis of connected volumes: scatter plot $ta$ vs. $\theta$:
    \begin{itemize}
        \item binning of data (porosity ranges) allows to determine statistics of $ta$ for every value range of porosity
        \item statistical check using normality tests on data and log-transformed data
        \item for low porosities, (below mean porosity value) the $ta$ shows clearly log-normal distribution properties, i.e. in normal scale skewed distribution with ail towards very low $ta$ value; 
        \item interpretation: for low porosities the structure/ distrbution of void space is crucial for $ta$; stronger differences given large differences possible in structure of void space: i.e. single wide flow channel almost like plug flow (high $ta$), whereas hardly connected domain with bottleneck shaped passages hampers transport; thus large spread of possible $ta$ values with significant tail of low $ta$ values referring to domains which are hardly connected 
        \item log-normal distribution relates well to averaging behaviour of flow in networks: for random networks the geometric mean is the representative value (similar in Darcy flow settings, refer to stochastic hydrogeology)
        \item for higher porosities, the distribution of $ta$ values shows stronger normality
        \item interpretation: the higher the porosity the more connected pathways through the network. The differences in the structure between individual small volumes reduces, and impact of void space structure is less. Thus, differences in the transport ability reduces.
        \item functional description of log-normal $ta$ with characterising parameters as function of porosity value $q_1(\theta)$ and $q_2(\theta)$ --> Figure for "observed" $ta$ - values
        \item parameters meaning: $q_1(\theta)$ refers to geometric mean value, whereas $q_2(\theta)$ refers to log-$ta$ std/variance 
        % \iten equation expression for connected $ta$: log-normal distribution:
    \end{itemize}
%    \iten equation expression for $ta$ (total) making use of $ta(\theta)$ and $p_con(\theta)$:
\end{itemize}

\section{Upscaling Procedure}

\subsection{Monte Carlo Simualtions: numerical upscaling}
\begin{itemize}
    \item create a figure: 4x4 network, $\theta$-values (random), $ta$ values random (including black elements for non-connected elements)
    \item defining network of 4x4 elements (or larger network for choice of upscaling domain)
    \item generate random porosity values: 
        \begin{itemize}
            \item sampling from normal distribution with mean and variance according to spatial scale; 
            \item 4 elements share the same value due to spatial correlation
            \item mean porosity of network $\bar \theta$ is arithmetic average of individual values; 
            \item grouping of 4 ensures that average porosities (of an ensemble of networks) follows statistics determined for data
        \end{itemize}
    \item generate transport ability from porosity values: (a) connection
        \begin{itemize}
            \item calculated probability of connectivity for every network element from connectivity function 
            \item random sampling of uniform distributed value $v$ between 0 and 1 for every element --> if $p_con < v$ then element is not connected, otherwise connected
            \item non-connected values are assigned a $ta$ value of zero.
        \end{itemize}
    \item generate transport ability from porosity values: (b) ta for connected value
        \begin{itemize}
        \item for every element the $ta$ value is sampled form the distribution which refer to its porosity values
        \item for every porosity value a histogram of $ta$ values is available; $ta$ values are randomly sampled from this distribution (using a python routine "sample from histogram"), thus the random $ta$ values are fully in line with observed values and no stochastic distribution is imposed.
        % \item log-normal distribution of $ta$ values
        \end{itemize}
    \item effective $ta$ value for network from flow simulation:
    \begin{itemize}
        \item a concentration gradient is imposed on both sides of the network domain
        \item the flux is calculated numerically solving the matrix equation for the flow system (where the adjacency matrix is build according the $ta$ values)
        \item $\bar ta_{eff}$ is calculated as ratio of the imposed concentration gradient and the calculated flux
    \end{itemize}
    \item for every network configuration: ensemble of $10000$ realizations, to analyse statistics of upscaled $\bar \theta$ and $ta_{eff}$ values:
        \begin{itemize}
            \item $2 \rightarrow 8 \mu m$
            \item $8 \rightarrow 32 \mu m$
            \item $2 \rightarrow 32 \mu m$
        \end{itemize}
    \item repetition of upscaling procedure with modification of connected $ta$ sampling using log-normal distribution instead of sample distribution to check applicability of stochastic $ta$ description
\end{itemize}

\subsection{Theoretical Upscaling}
\begin{itemize}
    \item statistical descriptions of porosity, connectivity and connected $ta$ allow for theoretical upscaling of $ta$ values:
    \item probability distribution for total $ta$ as function of porosity $\theta$ (making use of distribution functions and functional expressions): equation expression and Figure for $2 \mu m$
    \item warning: theoretical value refers to ergodic conditions which are not reached for network sizes (sub-REV)
    \item ToDo: upscaling by calculating expectation value and variance of $ta$ using mathematical definition: statistical expression and Figures
    % \item functional description of log-normal $ta$ with characterising parameters as function of porosity value $q_1(\theta)$ and $q_2(\theta)$ --> Figure for "observed" $ta$ - values
    % \item parameters meaning: $q_1(\theta)$ refers to geometric mean value, whereas $q_2(\theta)$ refers to log-$ta$ std/variance 
\end{itemize}

\section{Results and Discussion}
\begin{itemize}
    \item statistics of samples/upscaled porosity: is consistent with statistics of data
    \item statistics of numerically upscaled network $ta_{eff}$ at different scales:
        \begin{itemize}
            \item from 2 to 8 $\mu m$
            \item from 8 to 32 $\mu m$
            \item from 2 to 32 $\mu m$
        \end{itemize}
    \item scatter plot: $ta_G$ vs. $ta_{eff}$ 
    \item $ta_G$ is theoretical prediction for fully connected network (data analysis confirms directly correlation)
    \item upscaled  $ta_{eff}$ also reveal log-normal distribution with characterising parameters as function of porosity value: Figure with characterising parameters as function of porosity for different upscaling regimes
    \item theoretical upscaling expression in line with monte carlo?
    \item interpretation regarding generality of stochastic relation of $ta$ as function of $\theta$
    \item interpretation regarding convergence to larger averaging volumes: what happens when std of porosity is quasi zero, final $ta$ distribution, what is the required volume/area to average over (considering setting of this material)
\end{itemize}

\section{Conclusions}
\begin{itemize}
    \item non-uniformity of porosity is significant at sub-REV scale
    \item convergence of porosity to representative average value with increasing volume average hampers by spatial correlation of porosity
    
\end{itemize}

\begin{itemize}
    \item 
\end{itemize}

% Research Aim
% \begin{itemize}
%     \item derive relationship of permeability (transport ability) as function of porosity (taking percolation and not ergodicity into account), provide insight for mean and deviation behaviour 
% \end{itemize}

% Conceptual steps
% \begin{itemize}
%     \item starting point: porosity (not constant but statistically expressed)
%     \item 
% \end{itemize}

==> Figures.tex <==


\begin{figure}
\centering
    \includegraphics[width=0.45\textwidth]{Figures/TR_Histogram_ptotal_016_n2.png}
    \includegraphics[width=0.45\textwidth]{Figures/TR_Histogram_ptotal_034_n2.png}
\caption{Transport resistance distributions for total porosity in comparison to percolating porosity for two value of $\epsilon$: Frequency distribution of data (in green and yellow) and associated log-normal distribution (red and blue lines). (Porosity mean and standard deviation of particle 1 of FFC2 in resolution $n=2\,\mu$m.)}
    % \label{fig:stats_normal}
\end{figure}

